Adversarial Feedback Loop

Thanks to their remarkable generative capabilities, GANs have gained great popularity, and are used abundantly in state-of-the-art methods and applications. In a GAN based model, a discriminator is trained to learn the real data distribution. To date, it has been used only for training purposes, where it's utilized to train the generator to provide real-looking outputs. In this paper we propose a novel method that makes an explicit use of the discriminator in test-time, in a feedback manner in order to improve the generator results. To the best of our knowledge it is the first time a discriminator is involved in test-time. We claim that the discriminator holds significant information on the real data distribution, that could be useful for test-time as well, a potential that has not been explored before. The approach we propose does not alter the conventional training stage. At test-time, however, it transfers the output from the generator into the discriminator, and uses feedback modules (convolutional blocks) to translate the features of the discriminator layers into corrections to the features of the generator layers, which are used eventually to get a better generator result. Our method can contribute to both conditional and unconditional GANs. As demonstrated by our experiments, it can improve the results of state-of-the-art networks for super-resolution, and image generation.

==> fig_Table_CIFAR10.tex <==
\begin{figure*}
% \centering
\begin{subfigure}[b]{0.48\linewidth}
%  \centering
  \includegraphics[width=0.9\linewidth]{figs/inception_figure.pdf} 
  \label{fig:sub1}
\end{subfigure}%\hspace{5mm}
\begin{subfigure}[b]{.48\textwidth}
  \setlength{\tabcolsep}{.0em}
  \begin{tabu}{@{}lcccc@{}}
      \toprule
	\textbf{Method} & \phantom{ab} &  \textbf{Baseline} & \phantom{ab} & \textbf{Baseline+AFL(ours)}\\
    \midrule
        Weight clipping \cite{arjovsky2017wasserstein} && $6.41\pm.11$ && \\
        DCGAN \cite{radford2015unsupervised}(in \cite{yang2017lr}) && $6.64\pm.14$ && $\textbf{7.02}\pm.06$ \\
        WGAN-GP\cite{gulrajani2017improved} && $6.68\pm.06$ && {$\textbf{7.17}\pm.05$}\\
        Improved GAN \cite{salimans2016improved} && $6.86\pm.06$ && \\
        Layer Norm. \cite{ba2016layer} && $7.19\pm.12$ && \\
        Orthonormal \cite{brock2016neural}&& $7.40\pm.12$ && \\
        SN-GAN \cite{miyato2018spectral} && $7.42\pm.08$ && {$\textbf{7.73}\pm.05$} \\
        DFM \cite{warde2016improving}&& $7.72\pm.13$ && \\
    % \end{tabular}
        \bottomrule
    \end{tabu}
  \label{fig:sub2}
\end{subfigure}
\caption{\textbf{Image generation with AFL:} Inception Scores of several recent methods in unsupervised image generation on CIFAR-10. Combining our proposed AFL (in orange) with any one of three baselines improves the scores significantly.
\firas{should decide and update}}
\label{fig:Inception}
\end{figure*}
